COVID-19 in differential diagnosis of online symptom assessments

The COVID-19 pandemic has magnified an already existing trend of people looking for healthcare solutions online. One class of solutions are symptom checkers, which have become very popular in the context of COVID-19. Traditional symptom checkers, however, are based on manually curated expert systems that are inflexible and hard to modify, especially in a quickly changing situation like the one we are facing today. That is why all COVID-19 existing solutions are manual symptom checkers that can only estimate the probability of this disease and cannot contemplate alternative hypothesis or come up with a differential diagnosis. While machine learning offers an alternative, the lack of reliable data does not make it easy to apply to COVID-19 either. In this paper we present an approach that combines the strengths of traditional AI expert systems and novel deep learning models. In doing so we can leverage prior knowledge as well as any amount of existing data to quickly derive models that best adapt to the current state of the world and latest scientific knowledge. We use the approach to train a COVID-19 aware differential diagnosis model that can be used for medical decision support both for doctors or patients. We show that our approach is able to accurately model new incoming data about COVID-19 while still preserving accuracy on conditions that had been modeled in the past. While our approach shows evident and clear advantages for an extreme situation like the one we are currently facing, we also show that its flexibility generalizes beyond this concrete, but very important, example.

==> images/teximage.tex <==
\frame{\begin{picture}(100,100)
\put(25,50){\dashbox{.5}(10,10){$A$}}
\put(50,50){\dashbox{.5}(10,10){$B$}}
\end{picture}}


==> sections/model.old.tex <==
\section{Model}
\label{sec:model}
We are interested in building a machine learned model that takes findings as input, and outputs a ranked list of possible conditions (\emph{a.k.a.} differential diagnosis). We formulate this as a classification task, and use the output scores from the model to rank the conditions in the differential diagnosis. 

Let  $\mathcal{F} = \{f_1, \cdots , f_K\}$ be the universe of all the findings that can be elicited from the patients. Examples of findings include `eye pain', `nausea' and `fever'.  Let $\mathcal{Y} =  \{1, ..., L\}$ correspond to $L$ diagnoses that are of interest. Examples of diagnoses include `COVID-19', `arthritis' and `common cold'. 

A clinical case consists of (a) a set of findings $\mathbf{x}_{pos} \in \mathcal{F}$ that are observed in the patient; (b) a disjoint set of  findings $\mathbf{x}_{neg} \in \mathcal{F}$ that are explicitly observed to be not present in the patient; and (c) the corresponding differential diagnoses $\mathbf{ddx}$ such that  $\mathbf{ddx} = \{y_j \in \mathcal{Y}, s_j\}_{j=1}^{j=L}$, where $s_j$ (with  $\sum_j s_j = 1$) is the  probability of $y_j$ to be considered the true underlying diagnosis. We also assume that demographic variables such as gender and age are also part of $\mathbf{x}_{pos}$. Clearly,  $\mathbf{x}_{pos} \cap \mathbf{x}_{neg} = \emptyset$. While one may argue that all findings that are not present in the patient are therefore absent, in reality, the doctors gather information that are pertinent to the observed findings so as to rule-out possibly related diseases. In order to mimic this, we make the assumption that  $|\mathbf{x}_{pos} \cup \mathbf{x}_{neg} | << |\mathcal{F}|$.

\TODO{Finally, the model proposed in this paper directly operates on the findings/symptoms observed to be either positive or negative, while previous work uses tokens in findings as input vocabulary.}

We assume access to a labeled data set of $N$ clinical cases, $\mathcal{D} = \{(\mathbf{x}_{pos}^{(1)}, \mathbf{x}_{neg}^{(1)}, \mathbf{ddx}^{(1)}), \cdots ,(\mathbf{x}_{pos}^{(N)}, \mathbf{x}_{neg}^{(N)}, \mathbf{ddx}^{(N)})$. 
\\

\noindent {\bf Probabilistic cross-entropy loss}: 
The goal is to learn a function from $g: \mathcal{X} \mapsto \mathcal{Y}$ that minimizes empirical risk:
\begin{equation}
  \min_{g \in \mathcal{G}} \sum_{n=1}^{N} \textrm{loss}(\mathbf{ddx}^{(n)}, g(\mathbf{x}^{(n)}))
 \label{eqn:loss}
\end{equation}
where $ \textrm{loss}$ measures the discrepancy between the true label distribution  $\mathbf{ddx}^{(n)}$ and the predicted distribution $ g(\mathbf{x}^{(n)})$.  During evaluation we use 0/1 loss and during training, we use the surrogate \emph{soft} cross entropy loss between encoding of $y_n$ as a probability distribution and the output softmax probability vector provided by the function $g$. % so that:
%\begin{equation}
 %   \textrm{loss}(\mathbf{ddx}, g(\mathbf{x})) = \sum_{l=1}^{L} s_l \log g(\mathbf{x})[l], 
%\end{equation}
%where $g(\mathbf{x})[l]$ is the model's predicted score for class $l$.


%\begin{figure}
 % \centering
 % \includegraphics[scale=0.25]{figs/model.png}
 % \caption{Model Architecture used in learning to diagnose}
 % \label{fig:model}
%\end{figure}

 %It is  trained to minimize the soft cross-entropy between the predicted softmax distribution and the target distribution of each clinical case.
\noindent {\bf Loss:} In a typical classification cross entropy loss, the target is a vector with one non-zero entry corresponding to the ground truth label. However, often in clinical diagnosis setting, there is always some amount of uncertainty in the final diagnosis. As an example, for a patient with ``cough'', there are many possible diseases to be considered with some diseases such as ``common cold' or `flu' having a higher probability than diseases such as `pneumonia'.  In order to capture this, the target vector is a distribution over the plausible diagnoses, where the probability is based on the scores associated with the differential diagnoses. In \cite{mahajan18}, a similar construct was used in the context of image classification but assumed a uniform distribution over the target labels, and hence set the target to 1/k corresponding to the $k \ge 1$ labels for the image.

We acknowledge that even though the loss function models the entire differential diagnosis, we would ideally have a loss function that is cost-sensitive. For instance, misdiagnosing a disease that needs urgent care can lead to worse outcomes than misdiagnosing a common cold. This risk in misdiagnosis should ideally be taken into account.


%The model $g(\mathbf{x})$ provides probabilities over all diagnoses in the vocabulary using a softmax activation. 

\noindent {\bf Model: Functional form of g(\bf{x})}: Fig.~\ref{fig:model} provides an overview of the model for computing $g(\mathbf{x})$  in eqn.~\ref{eqn:loss}  . The model takes as input $\mathbf{x}_{pos}, \mathbf{x}_{neg}$ and predicts a distribution over the diagnosis. The model has separate input streams for the demographic variables and the findings.  Demographic variables include gender and age. They  impose an implicit prior over diseases that are impossible. As examples, it is impossible for a biologically male patient to be diagnosed with `pregnancy'. Similarly, its unlikely for an infant to be diagnosed with `dementia'. Incorporating these medically grounded priors into the model can facilitate faster model training as they can serve as the bottle neck over possible diagnoses. To reuse the `pregnancy' example, in the early iterations of training, a male patient with nausea and vomiting can be forced to have `zero' probability mass over women-related health issues, thereby greatly reducing the parameter search space. To model this, the embedding layers of demographic variables are assumed to be independent, and they have their separate $L$-dimensional space. The $L$ dimensional embedding vector is used to capture the prior probabilities of these variables to the set of $L$ diagnoses. We assume equal prior over all diseases that are plausible for a demographic variable. During training, the embeddings of the demographic variables are updated to learn better representations. 
 
We use separate embeddings for presence and absence of findings; the presence of a finding has a distinct role to play than its absence.  We use an embedding space of high dimensionality, followed by dropout for regularization, and then averaged and projected to a fully connected layer and a log-softmax activation function.  As we can see from the model architecture (Fig.~\ref{fig:model}), the demographic variable encodings are combined additively with the averaged embedding of the findings after a logsoftmax transformation. This enables the bottleneck property/role that we described above.




---------
\begin{table}[h]
\centering
\begin{tabular}{|l|}
\hline
\begin{minipage} [t]  {\textwidth} 
   \begin{itemize}[leftmargin=*]
\item in China in the past 14 days prior to symptoms onset
\item in Europe in the past 14 days prior to symptoms onset
\item in Iran in the past 14 days prior to symptoms onset
\item in Japan in the past 14 days prior to symptoms onset
\item dyspnea at rest
\item hospital personnel
\item exposure to COVID- 2019 within the last 14 days from symptom onset
\item healthcare contact with confirmed COVID-19 case not using any personal protective equipment
\item household contact with confirmed COVID-19 case
\item prolonged exposure to person with confirmed COVID-19 case (but not close contact)
\item recent close contact with a person with symptomatic confirmed COVID-19 case
   \end{itemize} 
\end{minipage} \\ \vspace*{0.1pt}\\ [3pt]  \hline  
\end{tabular}
\caption{Findings unique to COVID-19 assessment data, in comparison to dataset from the expert system (see section "Dataset from expert systems"}
\label{tbl:covidFindings}
\vspace{-10pt}
\end{table}

==> sections/overview.tex <==







%Unlike previous approaches, the proposed model is trained with a novel objective that takes into account the differential diagnosis of the clinical case, and not just a single disease.
%The proposed model is trained with an objective that takes into account the differential diagnosis of the clinical case, and not just a single disease.  With our proposed model, we combine the best of both worlds: a very focused COVID-19 assessment tool to capture the changing guidelines and known medical evidence for COVID-19 (eg. incorporating anosmia as a new finding), and the generality of a symptom checker that understands many other conditions besides COVID-19. The duality of the approach allows the consideration of COVID-19 in a differential diagnosis whenever appropriate while also modeling the probabilities of competing hypothesis. This paper extends the work of \cite{ravuri18} in multiple directions. To the best of our knowledge, this paper is the first in incorporating COVID-19 as part of the differential diagnosis for an automated diagnosis assessment. Another difference to pre-existing work, that is particularly relevant for COVID-19, is that in this work we combine the data from the expert system with a snapshot of a dataset collected from an online COVID-19 assessment tool, as opposed to e.g. data from EHRs. In a rapidly evolving situation like the one we face today, data from EHR is still noisy and incomplete. Using data from a specific online assessment tool is a novel approach to not only quickly generate data, but also to incrementally improve it over time as new information about the condition is uncovered and added to the assessment. Finally, the model proposed in this paper directly operates on the findings/symptoms observed to be either positive or negative, while previous work uses tokens in findings as input vocabulary.







==> sections/related.tex <==
%\begin{itemize}
%\item Online symptom checkers
%\item Differential diagnosis
%\item covid specific
%\end{itemize}

%\begin{figure*}
%  \centering
%  \includegraphics[width=.75\linewidth]{figs/simulator_model.png}
%  \caption{(a) Expert systems as prior: Describes the flow of data generation that can used to train model (b) Examples
%  of differential diagnosis inferred from expert systems, classification model trained from expert systems and after 
%  incorporating COVID cases \TODO{update the diagram}}
 % \label{fig:prior}
%\end{figure*}


\section{Related work}
\noindent\textbf{Differential diagnosis  as Inference:} Early models for diagnosis were AI expert system models used as medical decision support systems for physicians ({\it c.f.} Mycin~\cite{mycin}, Internist-1~\cite{miller_internist-1_1982}, DXplain~\cite{barnett_dxplain:_1987} and QMR~\cite{rassinoux_modeling_1996}). The goal of these systems was to emulate physicians' medical diagnostic ability to provide an ``independent expert opinion'' that could be leveraged by physicians when making a final decision.  These systems have two components: an expert-curated knowledge base and an inference engine that is manually optimized. A fundamental limitation of these approaches and their probabilistic counterparts (c.f.\cite{ShweCooper90, Morris01})
is the \emph{knowledge acquisition} problem \cite{gaines_knowledge_2013, Miller1986TheIM}:   the knowledge base construction is time-consuming. Adding an extra disease requires weeks of work from expert physicians who need to corroborate evidences from multiple peer-reviewed publications and other sources. 

\noindent\textbf{Machine learned models}
Machine learning provides a viable scalable path to quickly learn (and revise) models of differential diagnosis, as they depend on patient-level data available from sources such as electronic health records. While the initial work in this space has been on learning diagnostic codes (ICD) predictions using deep neural networks, either instantaneously or through time (\emph{c.f.} \cite{miotto_deep_2016, Ling_DeepRL_Diagnostic, Shickel_Deep_EHR, Rajkomar18, liang2019} and references therein), more recently, \cite{ravuri18, kannan20}, these approaches have been applied to directly modeling the task of coming up with a differential diagnosis in a manner that is useful in patient-facing settings such as online symptom checkers. Ravuri et al. \cite{ravuri18} also introduce the idea of using expert systems as a data prior which forms the basis of our current work. 


To the best of our knowledge, our approach is the first to incorporate COVID-19 as part of the differential diagnosis for an automated diagnosis assessment. Another difference to pre-existing work such \cite{ravuri18, kannan20} is that we combine data from the expert system with a snapshot of a dataset collected from an online COVID-19 assessment tool, as opposed to e.g. data from EHRs.  In a rapidly evolving situation like the one we face today, data from EHR is still noisy and incomplete and is not easily available. Using data from a specific online assessment tool is a novel approach because (a) we get patient data on their symptoms and (b) assessment tool itself is incrementally improved over time as new information about the condition emerges, and thus observational data from patients is up-to-date. 






==> sections/semigran.tex <==

\begin{table*}[h]
\centering
\tiny
\begin{tabular}{lllll}
\toprule
Findings   & Label  & \Base & \BaseCOVID  & \BaseCOVIDFULL  \\ 
\hline
female &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
  {\bf acute liver failure} (0.23) &
 {\bf acute liver failure} (0.24) &
  {\bf acute liver failure} (0.31) \\
drowsiness &
   &
  hepatic encephalopathy (0.14) &
  hepatic encephalopathy (0.15) &
  opioid intoxication (0.1) \\
right upper abdominal tenderness &
   &
  salicylate toxicity (0.12) &
  salicylate toxicity (0.14) &
  hepatic encephalopathy (0.09) \\
acetaminophen ingestion &
  acute liver failure &
  opioid intoxication (0.1) &
  opioid intoxication (0.1) &
  salicylate toxicity (0.09) \\
consciousness disturbance &
   &
  diabetic ketoacidosis (0.09) &
  diabetic ketoacidosis (0.05) &
  obstructive sleep apnea (0.05) \\
delirium &
   &
   &
   &
   \\
 \hline
female &
   &
   &
   &
   \\
adolescent ($\sim$12 to \textless 18 yrs) &
   &
   &
   &
   \\
abdominal pain &
   &
  viral gastroenteritis (0.8) &
  viral gastroenteritis (0.81) &
  viral gastroenteritis (0.84) \\
sudden onset &
   &
  intestinal obstruction (0.13) &
  intestinal obstruction (0.11) &
  intestinal obstruction (0.09) \\
nausea &
  appendicitis &
  salmonella food poisoning (0.01) &
  salmonella food poisoning (0.01) &
  acute mesenteric vascular insufficiency (0.02) \\
vomiting &
   &
  acute mesenteric vascular insufficiency (0.01) &
  acute mesenteric vascular insufficiency (0.01) &
  salmonella food poisoning (0.01) \\
diarrhea &
   &
  influenza (0.01) &
  influenza (0.01) &
  influenza (0.01) \\
high fever (\textgreater{}104 \& \textless 106.7F) &
   &
   &
   &
   \\
\hline
female &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
asthma &
   &
  {\bf asthma} (1.0) &
  {\bf asthma} (1.0) &
  {\bf asthma} (1.0) \\
respiratory distress &
   &
  chronic bronchitis (0.0) &
  chronic bronchitis (0.0) &
  chronic bronchitis (0.0) \\
dyspnea &
  asthma exacerbation &
  acute bronchitis (0.0) &
  acute bronchitis (0.0) &
  acute bronchitis (0.0) \\
wheezing &
   &
  generalized anaphylaxis (0.0) &
  generalized anaphylaxis (0.0) &
  generalized anaphylaxis (0.0) \\
cough &
   &
  aspiration pneumonia (0.0) &
  aspiration pneumonia (0.0) &
  aspiration pneumonia (0.0) \\
recent illness &
   &
   &
   &
   \\
\hline
female &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
  {\bf chronic bronchitis} (0.8) &
  {\bf chronic bronchitis} (0.78) &
  {\bf chronic bronchitis} (0.74) \\
chronic obstructive pulmonary disease &
   &
  bacterial pneumonia (0.13) &
  bacterial pneumonia (0.16) &
  bacterial pneumonia (0.2) \\
progressive dyspnea &
   &
  acute bronchitis (0.03) &
  acute bronchitis (0.03) &
  acute bronchitis (0.03) \\
productive cough &
  COPD exacerbation &
  pulmonary embolism (0.01) &
  pulmonary embolism (0.01) &
  pulmonary embolism (0.01) \\
purulent sputum &
   (pulmonary emphysema, &
  idiopathic pulmonary fibrosis (0.01) &
  idiopathic pulmonary fibrosis (0.0) &
  asthma (0.0) \\
low grade fever (100.4 - 100.9F) &
   chronic bronchitis) &
   &
   &
   \\
\hline
female &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
unilateral lower extremity edema &
   &
  {\bf deep vein thrombosis} (0.93) &
  {\bf deep vein thrombosis} (0.89) &
  {\bf deep vein thrombosis} (0.91) \\
lower extremity tenderness &
   &
  stasis dermatitis (0.02) &
  stasis dermatitis (0.03) &
  stasis dermatitis (0.02) \\
lower extremity erythema &
  deep vein thrombosis &
  inherited thrombophilia (0.01) &
  inherited thrombophilia (0.02) &
  inherited thrombophilia (0.01) \\
recent hospitalization &
   &
  pulmonary embolism (0.01) &
  pulmonary embolism (0.01) &
  postphlebitic syndrome (0.01) \\
lower extremity pain &
   &
  postphlebitic syndrome (0.01) &
  postphlebitic syndrome (0.01) &
  pulmonary embolism (0.01) \\
%symptoms started within the last several days (\textgreater{}2 days \& \textless{}8 days) &
   &
   &
   &
   \\
\hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
substernal chest pain &
   &
  {\bf acute myocardial infarction} (0.66) &
  {\bf acute myocardial infarction} (0.79) &
  {\bf acute myocardial infarction} (0.73) \\
diaphoresis &
   &
  angina pectoris (0.18) &
  angina pectoris (0.11) &
  angina pectoris (0.15) \\
hyperhidrosis &
  acute myocardial infarction &
  pulmonary embolism (0.16) &
  pulmonary embolism (0.09) &
  pulmonary embolism (0.11) \\
respiratory distress &
   &
  dissecting aortic aneurysm (0.01) &
  dissecting aortic aneurysm (0.01) &
  dissecting aortic aneurysm (0.01) \\
dyspnea &
   &
  hyperventilation syndrome (0.0) &
  hyperventilation syndrome (0.0) &
  asthma (0.0) \\
chest pressure &
   &
   &
   &
   \\
\hline
male &
   &
  salmonella food poisoning (0.53) &
  shigellosis (0.52) &
  salmonella food poisoning (0.39) \\
child (1 to $\sim$11 yrs) &
   &
  shigellosis (0.29) &
  salmonella food poisoning (0.31) &
  shigellosis (0.32) \\
abdominal pain &
  hemolytic-uremic syndrome &
  ulcerative colitis (0.17) &
  ulcerative colitis (0.16) &
  ulcerative colitis (0.27) \\
bloody diarrhea &
   &
  hemolytic-uremic syndrome (0.01) &
  hemolytic-uremic syndrome (0.01) &
  acute mesenteric vascular insufficiency (0.01) \\
meat ingestion &
   &
  acute mesenteric vascular insufficiency (0.01) &
  acute mesenteric vascular insufficiency (0.01) &
  hemolytic-uremic syndrome (0.01) \\
\hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
flank pain &
   &
  {\bf ureteral calculus} (0.78) &
   {\bf ureteral calculus} (0.77) &
  {\bf ureteral calculus} (0.77) \\
nausea &
   &
  acute pyelonephritis (0.12) &
  acute pyelonephritis (0.11) &
  acute pyelonephritis (0.13) \\
vomiting &
  nephrolithiasis  &
  acute appendicitis (0.02) &
  acute appendicitis (0.02) &
  acute appendicitis (0.01) \\
inguinal pain &
   (ureteral calculus) &
  primary hyperparathyroidism (0.01) &
  primary hyperparathyroidism (0.01) &
  primary hyperparathyroidism (0.01) \\
symptoms started within the last 6 hours &
   &
  carbon tetrachloride poisoning (0.01) &
  carbon tetrachloride poisoning (0.01) &
  carbon tetrachloride poisoning (0.01) \\
no positional change &
   &
   &
   &
   \\
\hline
male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
fever &
   &
   &
   &
   \\
chills &
   &
   &
   &
   \\
rigor &
   &
  dengue (0.48) &
  dengue (0.6) &
  dengue (0.45) \\
acute diarrhea &
   &
  Chikungunya virus infection (0.28) &
  Chikungunya virus infection (0.18) &
  Chikungunya virus infection (0.27) \\
foreign travel history &
  malaria &
  {\bf malaria} (0.13) &
  West Nile fever (0.1) &
  {\bf malaria}  (0.17) \\
mosquito bite &
   &
  West Nile fever (0.07) &
  {\bf malaria}  (0.07) &
  West Nile fever (0.07) \\
Central America &
   &
  yellow fever (0.02) &
  yellow fever (0.03) &
  yellow fever (0.02) \\
%symptoms started within the last several days (\textgreater{}2 days \& \textless{}8 days) &
   &
   &
   &
   \\
mosquito exposure &
   &
   &
   &
   \\
no quinacrine use &
   &
   &
   &
   \\
\hline
male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
  {\bf  bacterial meningitis} (0.87) &
 {\bf  bacterial meningitis} (0.73) &
  {\bf  bacterial meningitis} (0.78) \\
severe headache &
   &
  West Nile fever (0.1) &
  West Nile fever (0.24) &
  West Nile fever (0.18) \\
fever &
   &
  Rocky Mountain spotted fever (0.01) &
  Rocky Mountain spotted fever (0.02) &
  Rocky Mountain spotted fever (0.01) \\
photophobia &
  meningitis &
  influenza (0.0) &
  epidemic myalgic encephalomyelitis (0.0) &
  influenza (0.01) \\
nuchal rigidity &
   &
  epidemic myalgic encephalomyelitis (0.0) &
  influenza (0.0) &
  epidemic myalgic encephalomyelitis (0.0) \\
neck stiffness &
   &
   &
   &
   \\
\hline
male &
   &
  {\bf bacterial pneumonia} (0.53) &
  {\bf bacterial pneumonia} (0.6) &
  {\bf bacterial pneumonia} (0.55) \\
middle age (41 to 70 yrs) &
   &
  pulmonary embolism (0.14) &
  pulmonary embolism (0.13) &
  pulmonary embolism (0.15) \\
hypertension &
   &
  influenza (0.08) &
  influenza (0.1) &
  influenza (0.11) \\
osteoarthritis &
  pneumonia &
  primary gout (0.05) &
  congestive heart failure (0.02) &
  primary gout (0.05) \\
productive cough &
   &
  acute sinusitis (0.04) &
  acute sinusitis (0.02) &
  congestive heart failure (0.02) \\
fever &
   &
   &
   &
   \\
\hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
respiratory distress &
   &
  {\bf pulmonary embolism} (0.96) &
  {\bf pulmonary embolism}(0.95) &
  {\bf pulmonary embolism} (0.94) \\
dyspnea &
   &
  subacute bacterial endocarditis (0.01) &
  subacute bacterial endocarditis (0.01) &
  subacute bacterial endocarditis (0.02) \\
pleuritic chest pain &
   &
  deep vein thrombosis (0.01) &
  deep vein thrombosis (0.01) &
  deep vein thrombosis (0.01) \\
recent surgery &
  pulmonary embolism &
  bacterial pneumonia (0.01) &
  bacterial pneumonia (0.01) &
  bacterial pneumonia (0.01) \\
recent immobilization &
   &
  congestive heart failure (0.0) &
  congestive heart failure (0.0) &
  dissecting aortic aneurysm (0.0) \\
lower extremity tenderness &
   &
   &
   &
   \\
fever &
   &
   &
   &
   \\
unilateral lower extremity edema &
   &
   &
   &
   \\
\end{tabular}
\label{tbl:semigran2}
\caption{Results on \Semigran~ dataset. Please see rest of the clinical cases in the next few pages}
\end{table*}


\begin{table*}[h]
\centering
\tiny
\begin{tabular}{lllll}
\toprule
Findings   & Label  & \Base & \BaseCOVID  & \BaseCOVIDFULL  \\ 
\hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
nausea &
   &
  {\bf brain hemorrhage} (0.5) &
  {\bf brain hemorrhage} (0.5) &
  {\bf brain hemorrhage} (0.47) \\
vomiting &
   &
  glioblastoma (0.08) &
  glioblastoma (0.07) &
  glioblastoma (0.1) \\
 upper extremity muscle weakness &
  stroke &
  brain abscess (0.07) &
  brain abscess (0.07) &
  brain abscess (0.08) \\
dysarthria &
   (any type) &
  transient ischemic attacks (0.06) &
  transient ischemic attacks (0.06) &
  transient ischemic attacks (0.08) \\
aphasia &
   &
  bacterial meningitis (0.04) &
  bacterial meningitis (0.05) &
  botulism (0.04) \\
right upper extremity paralysis &
   &
   &
   &
   \\
\hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
difficulty opening mouth &
   &
   &
   &
   \\
trismus &
   &
  {\bf tetanus} (0.52) &
   {\bf tetanus}  (0.49) &
   {\bf tetanus}  (0.51) \\
diaphoresis &
   &
  gas gangrene (0.39) &
  gas gangrene (0.44) &
  gas gangrene (0.4) \\
hyperhidrosis &
   &
  Chinese restaurant syndrome (0.01) &
  Chinese restaurant syndrome (0.01) &
  serotonin syndrome (0.01) \\
tachycardia &
  tetanus &
  serotonin syndrome (0.01) &
  cellulitis (0.01) &
  Chinese restaurant syndrome (0.01) \\
laceration &
   &
  cellulitis (0.01) &
  serotonin syndrome (0.01) &
  cellulitis (0.01) \\
difficulty opening mouth &
   &
   &
   &
   \\
trismus &
   &
   &
   &
   \\
soil exposure &
   &
   &
   &
   \\
 \hline
female &
   &
   &
   &
   \\
infant (2 mo to \textless 1 yr) &
   &
   &
   &
   \\
serous nasal discharge &
   &
  adenovirus infection (0.61) &
  adenovirus infection (0.36) &
  adenovirus infection (0.46) \\
nasal discharge &
   &
  influenza (0.14) &
  influenza (0.18) &
  influenza (0.15) \\
cough &
   &
  acute sinusitis (0.1) &
  acute bronchitis (0.12) &
  acute sinusitis (0.12) \\
nasal congestion &
  acute otitis media &
  acute bronchitis (0.05) &
  COVID-19  (0.11) &
  acute bronchitis (0.08) \\
Irritable infant &
   &
  spasmodic croup (0.03) &
  acute sinusitis (0.07) &
  COVID-19 (0.05) \\
anorexia &
   &
   &
   &
   \\
fever &
   &
   &
   &
   \\
daycare attendance &
   &
   &
   &
   \\
  \hline
female &
   &
   &
   &
   \\
child (1 to $\sim$11 yrs) &
   &
   &
   &
   \\
fever &
   &
   &
   &
   \\
nausea &
   &
   &
   &
   \\
vomiting &
   &
  {\bf treptococcal pharyngitis} (0.93) &
  {\bf treptococcal pharyngitis}  (0.94) &
  {\bf treptococcal pharyngitis}  (0.93) \\
throat pain &
   &
  acute tonsillitis (0.03) &
  acute tonsillitis (0.02) &
  acute tonsillitis (0.03) \\
lymphadenopathy &
  streptococcal pharyngitis &
  infectious mononucleosis (0.01) &
  infectious mononucleosis (0.01) &
  infectious mononucleosis (0.01) \\
tonsillar exudate &
   &
  influenza (0.01) &
  influenza (0.01) &
  influenza (0.01) \\
no cough &
   &
  chronic pharyngitis (0.0) &
  chronic pharyngitis (0.0) &
  chronic pharyngitis (0.0) \\
no serous nasal discharge &
   &
   &
   &
   \\
no nasal discharge &
   &
   &
   &
   \\
no nasal congestion &
   &
   &
   &
   \\
   \hline
male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
  {\bf streptococcal pharyngitis}  (0.98) &
  {\bf streptococcal pharyngitis}  (0.98) &
  v (0.98) \\
throat pain &
   &
  infectious mononucleosis (0.01) &
  infectious mononucleosis (0.01) &
  acute tonsillitis (0.01) \\
fever &
   &
  acute tonsillitis (0.01) &
  acute tonsillitis (0.01) &
  infectious mononucleosis (0.01) \\
headache &
  streptococcal pharyngitis &
  peritonsillar abscess (0.0) &
  peritonsillar abscess (0.0) &
  peritonsillar abscess (0.0) \\
tonsillar exudate &
   &
  adenovirus infection (0.0) &
  adenovirus infection (0.0) &
  hand-foot-and-mouth disease (0.0) \\
no cough &
   &
   &
   &
   \\
   \hline
female &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
nasal congestion &
   &
  {\bf acute sinusitis} (0.63) &
  {\bf acute sinusitis}  (0.5) &
 {\bf acute sinusitis}  (0.53) \\
purulent nasal discharge &
   &
  chronic sinusitis (0.28) &
  chronic sinusitis (0.4) &
  chronic sinusitis (0.35) \\
unilateral purulent nasal discharge &
  acute sinusitis &
  cluster headache (0.02) &
  cluster headache (0.02) &
  cluster headache (0.04) \\
facial pain &
   &
  nasal foreign body (0.02) &
  nasal foreign body (0.02) &
  nasal foreign body (0.02) \\
no fever &
   &
  allergic rhinitis (0.01) &
  allergic rhinitis (0.01) &
  allergic rhinitis (0.01) \\
no chronic &
   &
   &
   &
   \\
   \hline
male &
   &
  cauda equina syndrome (0.35) &
  sciatic neuropathy (0.35) &
  cauda equina syndrome (0.38) \\
young adult (18 to 40 yrs) &
   &
  sciatic neuropathy (0.3) &
  cauda equina syndrome (0.33) &
  sciatic neuropathy (0.36) \\
back pain &
  lumbar intervertebral disc rupture &
  spinal cord compression (0.08) &
  spinal cord compression (0.08) &
  {\bf lumbar intervertebral disc rupture} (0.07) \\
foot drop &
   &
  {\bf lumbar intervertebral disc rupture} (0.08) &
  muscular low back pain (0.05) &
  spinal cord compression (0.05) \\
left foot drop &
   &
  muscular low back pain (0.04) &
  {\bf lumbar intervertebral disc rupture} (0.05) &
  muscular low back pain (0.03) \\
  \hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
lower extremity tenderness &
   &
  {\bf cellulitis} (0.52) &
   {\bf cellulitis} (0.51) &
   {\bf cellulitis} (0.39) \\
unilateral lower extremity edema &
   &
  deep vein thrombosis (0.21) &
  primary gout (0.18) &
  deep vein thrombosis (0.29) \\
lower extremity erythema &
  cellulitis &
  primary gout (0.16) &
  deep vein thrombosis (0.17) &
  primary gout (0.18) \\
low grade fever (100.4 - 100.9F) &
   &
  rheumatoid arthritis (0.02) &
  rheumatoid arthritis (0.04) &
  stasis dermatitis (0.03) \\
skin erythema &
   &
  stasis dermatitis (0.02) &
  stasis dermatitis (0.02) &
  rheumatoid arthritis (0.03) \\
lower extremity pain &
   &
   &
   &
   \\
   \hline
female &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
respiratory distress &
   &
  {\bf chronic bronchitis} (0.43) &
   {\bf chronic bronchitis}  (0.37) &
   {\bf chronic bronchitis} (0.41) \\
dyspnea &
   &
  bacterial pneumonia (0.22) &
  bacterial pneumonia (0.27) &
  bacterial pneumonia (0.27) \\
tobacco use disorder &
   &
  asthma (0.09) &
  asthma (0.08) &
  asthma (0.09) \\
productive cough &
  COPD exacerbation &
  pulmonary embolism (0.07) &
  pulmonary embolism (0.07) &
  pulmonary embolism (0.06) \\
serous nasal discharge &
   (pulmonary emphysema, &
  acute bronchitis (0.07) &
  acute bronchitis (0.07) &
  acute bronchitis (0.06) \\
nasal discharge &
   chronic bronchitis)&
   &
   &
   \\
white sputum &
   &
   &
   &
   \\
no chills &
   &
   &
   &
   \\
   \hline
female &
   &
  {\bf influenza} (0.63) &
   {\bf influenza} (0.56) &
   {\bf influenza} (0.56) \\
young adult (18 to 40 yrs) &
   &
  bacterial pneumonia (0.33) &
  bacterial pneumonia (0.4) &
  bacterial pneumonia (0.4) \\
fever &
   &
  pulmonary tuberculosis (0.01) &
  sarcoidosis (0.01) &
  pulmonary tuberculosis (0.01) \\
cough &
  influenza &
  sarcoidosis (0.01) &
  pulmonary tuberculosis (0.01) &
  sarcoidosis (0.01) \\
generalized weakness &
   &
  adenovirus infection (0.0) &
  acute bronchitis (0.01) &
  acute bronchitis (0.01) \\
no influenza vaccination &
   &
   &
   &
    \hline

\end{tabular}
\caption{Results on \Semigran~ dataset}
\label{tbl:semigran3}
\end{table*}

\begin{table*}[h]
\centering
\tiny
\begin{tabular}{lllll}
\toprule
Findings   & Label  & \Base & \BaseCOVID  & \BaseCOVIDFULL  \\ 
\hline
male &
   &
   &
   &
   \\
child (1 to $\sim$11 yrs) &
   &
  bacterial pneumonia (0.34) &
  bacterial pneumonia (0.4) &
  bacterial pneumonia (0.42) \\
asthma &
   &
  acute bronchitis (0.17) &
  asthma (0.18) &
  asthma (0.2) \\
productive cough &
   &
  acute sinusitis (0.16) &
  acute bronchitis (0.15) &
  acute bronchitis (0.11) \\
fever &
  pneumonia &
  asthma (0.15) &
  acute sinusitis (0.12) &
  acute sinusitis (0.11) \\
purulent sputum &
   &
  spasmodic croup (0.06) &
  influenza (0.06) &
  chronic bronchitis (0.06) \\
no anorexia &
   &
   &
   &
   \\
   \hline
male &
   &
   &
   &
   \\
adolescent ($\sim$12 to \textless 18 yrs) &
   &
   &
   &
   \\
nausea &
   &
 {\bf salmonella food poisoning} (0.46) &
   {\bf salmonella food poisoning}(0.35) &
   {\bf salmonella food poisoning} (0.42) \\
vomiting &
   &
  viral gastroenteritis (0.24) &
  viral gastroenteritis (0.28) &
  viral gastroenteritis (0.27) \\
diarrhea &
  salmonella food poisoning &
  shigellosis (0.13) &
  shigellosis (0.2) &
  shigellosis (0.14) \\
crampy abdominal pain &
   &
  intestinal obstruction (0.12) &
  intestinal obstruction (0.11) &
  intestinal obstruction (0.1) \\
abdominal tenderness &
   &
  acute giardiasis (0.01) &
  acute giardiasis (0.02) &
  acute giardiasis (0.01) \\
raw meat ingestion &
   &
   &
   &
   \\
no bloody diarrhea &
   &
   &
   &
   \\
   \hline
male &
   &
   &
   &
   \\
elderly (\textgreater 70 yrs) &
   &
   &
   &
   \\
right-sided chest pain &
   &
  {\bf herpes zoster} (0.99) &
   {\bf herpes zoster} (0.99) &
   {\bf herpes zoster} (0.99) \\
chest erythema &
   &
  Chinese restaurant syndrome (0.0) &
  contact dermatitis (0.0) &
  Chinese restaurant syndrome (0.0) \\
headache &
   &
  contact dermatitis (0.0) &
  Chinese restaurant syndrome (0.0) &
  contact dermatitis (0.0) \\
malaise &
  herpes zoster &
  herpes simplex (0.0) &
  herpes simplex (0.0) &
  herpes simplex (0.0) \\
localized vesicular rash &
   &
  chilblains (0.0) &
  smallpox (0.0) &
  smallpox (0.0) \\
skin burning sensation &
   &
   &
   &
   \\
%symptoms started within the last several days (\textgreater{}2 days \& \textless{}8 days) &
   &
   &
   &
   \\
localized red macules &
   &
   &
   &
   \\
   \hline
female &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
dysuria &
   &
   &
   &
   \\
overactive bladder &
   &
   &
   &
   \\
urinary urgency &
   &
  {\bf acute cystitis, female} (0.63) &
  {\bf acute cystitis, female}(0.57) &
  {\bf acute cystitis, female} (0.66) \\
increased urinary frequency &
   &
  urethritis, female (0.22) &
  urethritis, female (0.3) &
  urethritis, female (0.23) \\
sexually active &
   &
  chronic interstitial cystitis (0.05) &
  chronic interstitial cystitis (0.04) &
  chronic interstitial cystitis (0.03) \\
no fever &
  urinary tract infection &
  cystocele (0.01) &
  cystocele (0.01) &
  cystocele (0.01) \\
no chills &
   (simple cystitis or complicated UTI) &
  trichomonas vaginalis infection (0.01) &
  trichomonas vaginalis infection (0.01) &
  trichomonas vaginalis infection (0.01) \\
no nausea &
   &
   &
   &
   \\
no vomiting &
   &
   &
   &
   \\
no back pain &
   &
   &
   &
   \\
no vaginal discharge &
   &
   &
   &
   \\
no vaginal pruritus &
   &
   &
   &
   \\
   \hline
female &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
dizziness &
   &
  {\bf benign paroxysmal positional vertigo} (0.66) &
  {\bf benign paroxysmal positional vertigo}(0.63) &
  {\bf benign paroxysmal positional vertigo} (0.58) \\
sudden onset &
   &
  vestibular neuronitis (0.12) &
  vestibular neuronitis (0.12) &
  vestibular neuronitis (0.14) \\
recurrent &
   &
  migraine syndrome (0.03) &
  migraine syndrome (0.05) &
  transient ischemic attacks (0.04) \\
no unilateral hearing loss &
  benign paroxysmal positional vertigo &
  transient ischemic attacks (0.03) &
  transient ischemic attacks (0.03) &
  migraine syndrome (0.04) \\
no hearing loss &
   &
  motion sickness (0.01) &
  cluster headache (0.01) &
  motion sickness (0.01) \\
no tinnitus &
   &
   &
   &
   \\
no muscle weakness &
   &
   &
   &
   \\
no numbness &
   &
   &
   &
   \\
   \hline
female &
   &
  acute sinusitis (0.19) &
  acute sinusitis (0.19) &
  influenza (0.14) \\
young adult (18 to 40 yrs) &
   &
  asthma (0.14) &
  asthma (0.1) &
  acute sinusitis (0.14) \\
cough &
   &
  influenza (0.13) &
  influenza (0.1) &
  asthma (0.11) \\
recent illness &
  acute bronchitis &
  botulism (0.07) &
  bacterial pneumonia (0.08) &
  bacterial pneumonia (0.11) \\
recent viral illness &
   &
  chronic bronchitis (0.07) &
  acute suppurative otitis media (0.08) &
  acute suppurative otitis media (0.09) \\
no fever &
   &
   &
   &
   \\
   \hline
female &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
  {\bf acute bronchitis} (0.34) &
 {\bf acute bronchitis}  (0.42) &
  {\bf acute bronchitis}  (0.38) \\
cough &
   &
  acute sinusitis (0.21) &
  chronic bronchitis (0.17) &
  chronic bronchitis (0.18) \\
purulent sputum &
   &
  chronic bronchitis (0.18) &
  acute sinusitis (0.16) &
  bacterial pneumonia (0.16) \\
serous nasal discharge &
  acute bronchitis &
  adenovirus infection (0.11) &
  bacterial pneumonia (0.12) &
  acute sinusitis (0.14) \\
nasal discharge &
   &
  bacterial pneumonia (0.1) &
  adenovirus infection (0.05) &
  adenovirus infection (0.06) \\
no fever &
   &
   &
   &
   \\
   \hline
male &
   &
   &
   &
   \\
adolescent ($\sim$12 to \textless 18 yrs) &
   &
   &
   &
   \\
unilateral eye redness &
   &
 {\bf bacterial conjunctivitis} (0.5) &
  {\bf bacterial conjunctivitis} (0.51) &
{\bf bacterial conjunctivitis} (0.54) \\
bilateral red eyes &
   &
  inclusion conjunctivitis (0.2) &
  inclusion conjunctivitis (0.2) &
  inclusion conjunctivitis (0.2) \\
conjunctival erythema &
  acute conjunctivitis &
  vernal conjunctivitis (0.18) &
  vernal conjunctivitis (0.14) &
  vernal conjunctivitis (0.14) \\
eye discharge &
    (any conjuctivitis)& 
  chemical conjunctivitis (0.07) &
  chemical conjunctivitis (0.09) &
  chemical conjunctivitis (0.07) \\
unilateral eye discharge &
   &
  adult gonococcal conjunctivitis (0.06) &
  adult gonococcal conjunctivitis (0.06) &
  adult gonococcal conjunctivitis (0.05) \\
no eye pain &
   &
   &
   &
   \\
no photophobia &
   &
   &
   &
   \\
   \hline
male &
   &
  {\bf adenovirus infection} (0.65) &
   {\bf adenovirus infection} (0.48) &
   {\bf adenovirus infection}(0.57) \\
young adult (18 to 40 yrs) &
   &
  influenza (0.14) &
  influenza (0.14) &
  influenza (0.18) \\
throat pain &
  viral pharyngitis &
  infectious mononucleosis (0.08) &
  acute tonsillitis (0.12) &
  infectious mononucleosis (0.08) \\
headache &
   (common cold, &
  acute tonsillitis (0.07) &
  infectious mononucleosis (0.11) &
  acute tonsillitis (0.06) \\
cough &
  adenovirus infection) &
  streptococcal pharyngitis (0.03) &
 COVID-19 (0.07) &
 COVID-19 (0.04) \\
  \hline
male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
nasal congestion &
   &
   &
   &
   \\
chronic &
   &
  vernal conjunctivitis (0.54) &
  vernal conjunctivitis (0.47) &
  vernal conjunctivitis (0.59) \\
sneezing &
   &
  {\bf allergic rhinitis} (0.32) &
  {\bf allergic rhinitis}  (0.37) &
  {\bf allergic rhinitis}  (0.27) \\
nose pruritus &
   &
  inclusion conjunctivitis (0.02) &
  inclusion conjunctivitis (0.03) &
  inclusion conjunctivitis (0.03) \\
eye pruritus &
  allergic rhinitis &
  rosacea (0.01) &
  rosacea (0.02) &
  rosacea (0.01) \\
unilateral eye redness &
   &
  chemical conjunctivitis (0.01) &
  chemical conjunctivitis (0.01) &
  chemical conjunctivitis (0.01) \\
watery eye discharge &
   &
   &
   &
   \\
throat pruritus &
   &
   &
   &
   \\
atopic dermatitis &
   &
   &
   &
\end{tabular}
\caption{Results on \Semigran~ dataset}
\label{tbl:semigran4}
\end{table*}
\begin{table*}[h]
\centering
\tiny
\begin{tabular}{lllll}
\toprule
Findings   & Label  & \Base & \BaseCOVID  & \BaseCOVIDFULL  \\ 
\hline
male &
   &
   &
   &
   \\
child (1 to $\sim$11 yrs) &
   &
   {\bf Rocky Mountain spotted fever} (0.65) &
  {\bf Rocky Mountain spotted fever} (0.64) &
  {\bf Rocky Mountain spotted fever} (0.63) \\
fever &
   &
  influenza (0.08) &
  influenza (0.09) &
  influenza (0.09) \\
chills &
   &
  dengue (0.06) &
  dengue (0.09) &
  dengue (0.07) \\
joint pain &
  Rocky Mountain spotted fever &
  cellulitis (0.03) &
  cellulitis (0.03) &
  streptobacillary rat-bite fever (0.02) \\
wrist erythema &
   &
  streptobacillary rat-bite fever (0.02) &
  streptobacillary rat-bite fever (0.02) &
  cellulitis (0.02) \\
ankle erythema &
   &
   &
   &
   \\
     \hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
respiratory distress &
   &
  {\bf pulmonary embolism} (0.96) &
   {\bf pulmonary embolism}(0.95) &
   {\bf pulmonary embolism}(0.94) \\
dyspnea &
   &
  subacute bacterial endocarditis (0.01) &
  subacute bacterial endocarditis (0.01) &
  subacute bacterial endocarditis (0.02) \\
pleuritic chest pain &
   &
  deep vein thrombosis (0.01) &
  deep vein thrombosis (0.01) &
  deep vein thrombosis (0.01) \\
recent surgery &
  pulmonary embolism &
  bacterial pneumonia (0.01) &
  bacterial pneumonia (0.01) &
  bacterial pneumonia (0.01) \\
recent immobilization &
   &
  congestive heart failure (0.0) &
  congestive heart failure (0.0) &
  dissecting aortic aneurysm (0.0) \\
lower extremity tenderness &
   &
   &
   &
   \\
fever &
   &
   &
   &
   \\
unilateral lower extremity edema &
   &
   &
   &
   \\
     \hline

female &
   &
   &
   &
   \\
adolescent ($\sim$12 to \textless 18 yrs) &
   &
   &
   &
   \\
fever &
   &
   &
   &
   \\
fatigue &
   &
  streptococcal pharyngitis (0.56) &
  streptococcal pharyngitis (0.51) &
  streptococcal pharyngitis (0.46) \\
dysphagia &
   &
  {\bf infectious mononucleosis} (0.29) &
  {\bf infectious mononucleosis} (0.33) &
  {\bf infectious mononucleosis}(0.36) \\
odynophagia &
   &
  peritonsillar abscess (0.05) &
  peritonsillar abscess (0.08) &
  peritonsillar abscess (0.09) \\
lymphadenopathy &
  infectious mononucleosis &
  acute tonsillitis (0.03) &
  acute tonsillitis (0.02) &
  acute tonsillitis (0.02) \\
throat pain &
   &
  hand-foot-and-mouth disease (0.01) &
  acute HIV infection (0.01) &
  hand-foot-and-mouth disease (0.01) \\
pharyngeal exudate &
   &
   &
   &
   \\
%symptoms started within the last several days (\textgreater{}2 days \& \textless{}8 days) &
   &
   &
   &
   \\
generalized macular rash &
   &
   &
   &
   \\
     \hline

male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
  {\bf duodenal ulcer} (0.48) &
  acute esophagitis (0.57) &
  acute esophagitis (0.54) \\
upper abdominal pain &
   &
  acute esophagitis (0.47) &
  {\bf duodenal ulcer}(0.37) &
  {\bf duodenal ulcer} (0.42) \\
chronic &
   &
  Barrett's esophagus (0.04) &
  Barrett's esophagus (0.05) &
  Barrett's esophagus (0.03) \\
intermittent &
  peptic ulcer disease &
  chronic gastritis (0.0) &
  chronic gastritis (0.0) &
  chronic gastritis (0.0) \\
relieved with antacids &
  (duodenal or gasric ulcer) &
  stomach carcinoma (0.0) &
  acute gastritis (0.0) &
  stomach carcinoma (0.0) \\
pain relieved with food &
   &
   &
   &
   \\
     \hline

male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
serous nasal discharge &
   &
   &
   &
   \\
nasal discharge &
   &
   &
   &
   \\
throat pain &
   &
   &
   &
   \\
diaphoresis &
   &
  {\bf adenovirus infection} (0.42) &
  influenza (0.33) &
  influenza (0.37) \\
hyperhidrosis &
   &
  influenza (0.3) &
  {\bf adenovirus infection} (0.32) &
  {\bf adenovirus infection} (0.31) \\
headache &
   &
  acute sinusitis (0.04) &
  COVID-19 (0.06) &
  acute sinusitis (0.04) \\
productive cough &
  upper respiratory tract infection &
  streptococcal pharyngitis (0.03) &
  acute sinusitis (0.04) &
  bacterial pneumonia (0.03) \\
generalized muscle pain &
   (common cold, &
  bacterial pneumonia (0.03) &
  streptococcal pharyngitis (0.03) &
  streptococcal pharyngitis (0.03) \\
clear sputum &
   adenovirus infection)&
   &
   &
   \\
symptoms started within 6-48 hours &
   &
   &
   &
   \\
no fever &
   &
   &
   &
   \\
no nuchal rigidity &
   &
   &
   &
   \\
no neck stiffness &
   &
   &
   &
   \\
     \hline

male &
   &
  {\bf viral gastroenteritis} (0.28) &
 {\bf viral gastroenteritis}  (0.3) &
  {\bf viral gastroenteritis}  (0.4) \\
child (1 to $\sim$11 yrs) &
   &
  acute hepatitis B (0.24) &
  acute hepatitis B (0.27) &
  acute hepatitis B (0.19) \\
low grade fever (100.4 - 100.9F) &
  gastroenteritis &
  acute hepatitis D (0.14) &
  acute hepatitis D (0.18) &
  acute hepatitis D (0.1) \\
vomiting &
   &
  acute appendicitis (0.08) &
  acute appendicitis (0.06) &
  acute appendicitis (0.05) \\
    \hline

male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
low back pain &
   &
  {\bf muscular low back pain} (0.32) &
  {\bf muscular low back pain}(0.35) &
  {\bf muscular low back pain} (0.26) \\
no lower extremity pain &
   &
  sciatic neuropathy (0.18) &
  sciatic neuropathy (0.16) &
  sciatic neuropathy (0.21) \\
no lower extremity muscle weakness &
  low back strain &
  lumbar intervertebral disc rupture (0.07) &
  lumbar intervertebral disc rupture (0.05) &
  cauda equina syndrome (0.07) \\
no fever &
   &
  cauda equina syndrome (0.05) &
  cauda equina syndrome (0.05) &
  lumbar intervertebral disc rupture (0.07) \\
no chills &
   &
  dissecting aortic aneurysm (0.04) &
  dissecting aortic aneurysm (0.05) &
  dissecting aortic aneurysm (0.04) \\
no weight loss &
   &
   &
   &
   \\
no recent illness &
   &
   &
   &
   \\  \hline

male &
   &
   &
   &
   \\
child (1 to $\sim$11 yrs) &
   &
   &
   &
   \\
bee sting &
   &
  generalized anaphylaxis (0.37) &
  generalized anaphylaxis (0.46) &
  generalized anaphylaxis (0.37) \\
lip swelling &
   &
  herpes simplex (0.3) &
  herpes simplex (0.27) &
  herpes simplex (0.28) \\
lip tenderness &
  bee sting without anaphylaxis &
  {\bf hymenoptera sting} (0.12) &
  {\bf hymenoptera sting} (0.08) &
  {\bf hymenoptera sting} (0.11) \\
no tongue swelling &
   (hymenoptera sting)&
  allergic urticaria (0.09) &
  allergic urticaria (0.06) &
  allergic urticaria (0.09) \\
no drooling &
   &
  cholinergic urticaria (0.04) &
  cholinergic urticaria (0.04) &
  cholinergic urticaria (0.04) \\
no stridor &
   &
   &
   &
   \\
no rash &
   &
   &
   &
   \\
     \hline

male &
   &
   &
   &
   \\
adolescent ($\sim$12 to \textless 18 yrs) &
   &
   &
   &
   \\
oral ulcer &
   &
   &
   &
   \\
chronic &
   &
  hand-foot-and-mouth disease (0.19) &
  Behcet syndrome (0.24) &
  pemphigus vulgaris (0.35) \\
recurrent &
   &
  Behcet syndrome (0.18) &
  pemphigus vulgaris (0.19) &
  Behcet syndrome (0.16) \\
no skin lesion &
   &
  pemphigus vulgaris (0.17) &
  hand-foot-and-mouth disease (0.17) &
  hand-foot-and-mouth disease (0.15) \\
no medication use &
  recurrent aphthous stomatitis &
  streptococcal pharyngitis (0.09) &
  streptococcal pharyngitis (0.08) &
  streptococcal pharyngitis (0.07) \\
no illicit drug use &
   &
  allergic urticaria (0.03) &
  postphlebitic syndrome (0.04) &
  attention deficit hyperactivity disorder (0.04) \\
no anal ulceration &
   &
   &
   &
   \\
no gastrointestinal ulcer &
   &
   &
   &
   \\
no conjunctival ulcer &
   &
   &
   &
   \\
     \hline
female &
   &
  {\bf mycotic vulvovaginitis} (1.0) &
  {\bf mycotic vulvovaginitis} (0.99) &
  {\bf mycotic vulvovaginitis} (1.0) \\
young adult (18 to 40 yrs) &
   &
  trichomonas vaginalis infection, female (0.0) &
  trichomonas vaginalis infection, female (0.0) &
  trichomonas vaginalis infection, female (0.0) \\
vaginal pruritus &
   &
  diabetes mellitus in pregnancy (0.0) &
  diabetes mellitus in pregnancy (0.0) &
  diabetes mellitus in pregnancy (0.0) \\
cheesy vaginal discharge &
  candidal (mycotic) vulvovaginitis &
  diabetes mellitus type 1 (0.0) &
  diabetes mellitus type 1 (0.0) &
  diabetes mellitus type 1 (0.0) \\
no abdominal pain &
   &
  diabetes mellitus type 2 (0.0) &
  erythema multiforme (0.0) &
  diabetes mellitus type 2 (0.0) \\
no fever &
   &
   &
   &
   \\
\hline
\end{tabular}
\caption{Results on \Semigran~ dataset}
\label{tbl:semigran5}
\end{table*}

\begin{table*}[h]
\centering
\tiny
\begin{tabular}{lllll}
\toprule
Findings   & Label  & \Base & \BaseCOVID  & \BaseCOVIDFULL  \\ 
\hline
male &
   &
   &
   &
   \\
infant (2 mo to \textless 1 yr) &
   &
   &
   &
   \\
constipation &
   &
  {\bf constipation} (0.98) &
   {\bf constipation}  (0.98) &
   {\bf constipation}  (0.99) \\
hard stool &
   &
  perianal abscess (0.01) &
  perianal abscess (0.01) &
  perianal abscess (0.0) \\
painful bowel movement &
  acute constipation &
  ulcerative colitis (0.0) &
  anal fissure (0.0) &
  ulcerative colitis (0.0) \\
hematochezia &
   &
  anal fissure (0.0) &
  ulcerative colitis (0.0) &
  anal fissure (0.0) \\
infant diet change &
   &
  anorectal stricture (0.0) &
  anorectal stricture (0.0) &
  anorectal stricture (0.0) \\
no feeding problem of infant &
   &
   &
   &
   \\
     \hline

female &
   &
   &
   &
   \\
adolescent ($\sim$12 to \textless 18 yrs) &
   &
   &
   &
   \\
pruritic skin lesion &
   &
  adult hypothyroidism (0.31) &
  Sjogren syndrome (0.27) &
  adult hypothyroidism (0.19) \\
dry skin &
   &
  Sjogren syndrome (0.23) &
  adult hypothyroidism (0.19) &
  psoriasis (0.13) \\
scaly skin lesion &
  atopic dermatitis &
  psoriasis (0.13) &
  Stevens-Johnson syndrome (0.09) &
  Sjogren syndrome (0.12) \\
allergic rhinitis &
   (eczema) &
  Stevens-Johnson syndrome (0.07) &
  psoriasis (0.08) &
  {\bf eczema} (0.11) \\
allergy &
   &
  generalized anaphylaxis (0.04) &
  contact dermatitis (0.07) &
  Stevens-Johnson syndrome (0.08) \\
egg allergy &
   &
   &
   &
   \\
milk allergy &
   &
   &
   &
   \\
     \hline

male &
   &
   &
   &
   \\
young adult (18 to 40 yrs) &
   &
   &
   &
   \\
eyelid pain &
   &
  adult gonococcal conjunctivitis (0.34) &
  adult gonococcal conjunctivitis (0.39) &
  adult gonococcal conjunctivitis (0.3) \\
unilateral eyelid swelling &
   &
  inclusion conjunctivitis (0.21) &
  inclusion conjunctivitis (0.2) &
  inclusion conjunctivitis (0.21) \\
no traumatic injury &
   &
  {\bf external hordeolum} (0.1) &
  {\bf external hordeolum} (0.08) &
  nonulcerative blepharitis (0.1) \\
no visual impairment &
  external hordeolum &
  chemical conjunctivitis (0.08) &
  chemical conjunctivitis (0.08) &
  chemical conjunctivitis (0.09) \\
no eyelid crusting &
   &
  nonulcerative blepharitis (0.07) &
  nonulcerative blepharitis (0.06) &
   {\bf external hordeolum} (0.08) \\
no allergy &
   &
   &
   &
   \\
no unilateral eye pain &
   &
   &
   &
   \\
no unilateral eye redness &
   &
   &
   &
   \\
  \hline
male &
   &
   &
   &
   \\
middle age (41 to 70 yrs) &
   &
   &
   &
   \\
cough &
   &
  acute sinusitis (0.67) &
  acute sinusitis (0.61) &
  acute sinusitis (0.66) \\
sudden onset &
   &
  {\bf adenovirus infection} (0.2) &
  {\bf adenovirus infection} (0.16) &
 {\bf adenovirus infection} (0.15) \\
nasal congestion &
   &
  chronic sinusitis (0.06) &
  chronic sinusitis (0.09) &
  chronic sinusitis (0.1) \\
purulent nasal discharge &
  upper respiratory tract infection &
  influenza (0.04) &
  influenza (0.08) &
  influenza (0.04) \\
unilateral purulent nasal discharge &
    (common cold, &
  acute bronchitis (0.01) &
  acute bronchitis (0.02) &
  acute bronchitis (0.01) \\
low grade fever (100.4 - 100.9F) &
   common cold)&
   &
   &
   \\
serous nasal discharge &
   &
   &
   &
   \\
nasal discharge &
   &
   &
   &
\end{tabular}
\caption{Results on \Semigran~ dataset}
\label{tbl:semigran1}
\end{table*}

==> sections/side.tex <==
\begin{figure*}
\centering
\begin{minipage}{0.45\textwidth}
\centering
\begin{algorithm}[H]
\begin{algorithmic}[1]
\State {\bf Input}: Medical knowledge base of diseases ($\mathcal{D}$) and findings ($\mathcal{F}$) with relationships between them encoded by FREQ(d,f), where FREQ(d,f) is transformed to represent $p(f=1|d)$; number of cases T. Expert Inferene engine $ExpertInference$ that takes us input a set of findings and provides the differential diagnosis. 
\State {\bf Output}: $\{{\bf f}^{(t)}, {\bf ddx}^{(t)}\}_{t=1}^{T}$ pairs. such that $y \in \mathcal{D}$ and ${\bf f} \subset \mathcal{F}$ is the set of findings needed to arrive at {\bf ddx}. {\bf ddx} is differential diagnosis consisting of $K$ pairs of ( $y \in \mathcal{D}$, $s \in [0,1]$  such that  $\sum s_k = 1$  \\
\For{t = 1 to T} 
  \State  $y \sim  Uniform(\mathcal{D}^{*}) $ \Comment{Candidate disease label for this case}
  \State ${\bf f}^{(t)} \gets \emptyset$
  \State $F(*) = sort(\mathcal{F}, FREQ(y,:))$ \Comment{Findings sorted by frequency}
  \For{$f \in \textrm{Demographics}(\mathcal{F})$} \Comment{Demographic variables}
  	\If{$f \in F(*) \textrm{and rand()} > FREQ(f,y)$}
  	 	\State $ {\bf f}^{(t)} \gets {\bf f}^{(t)} \cup  \{f\}$
  	 	\State $F(*) \gets \textrm{RemoveMutex}(F(*) , {\bf f}^{(t)})$ \Comment{Remove all findings that can not co-manifest with ${\bf f}^{(t)}$}
     \EndIf
   \EndFor 
   \State L = randint(5, min(20, |F(*)|)) + $|  {\bf f}^{(t)}|$  \Comment{Sample a subset of findings}
   \State $F^{*} \gets  \mathcal{F} \setminus \textrm{Demographics}(\mathcal{F})$ 
    \While{ $| {\bf f}^{(t)}| \leq L $}
    	\State $F^{*} \gets \textrm{RemoveMutex}(F^{*}, {\bf f}^{(t)})$
    	\State $f^{*} \gets \textrm{GetNext}(F^{*})$ \Comment{Next finding to be visited}
        \If {$rand() > FREQ(f,y^{(t)})$}
    		\State $ {\bf f}^{(t)}  \gets {\bf f}^{(t)} \cup \{f^{*}\} $
            \State $F^{*} \gets F^{*} \setminus \{f^{*}\}$
 		\EndIf 
  	\EndWhile
  	\State  ${\bf ddx}^{(t)} \gets \textrm{ExpertInference}({\bf f}^{(t)})$ 
\EndFor
  \label{algo:generator}
 \end{algorithmic}
   \caption{Clinical case simulation algorithm }

\end{algorithm}
\cpation{figure caption goes here}\label{fig: figure-label}
\end{minipage}
\begin{minipage}}{0.45\textwidth}
\centering
\captionsetup{type=table} %% tell latex to change to table

\begin{table}[]
\centering
%\resizebox{\textwidth}{!}
{\begin{tabular}{ll}
\toprule
Findings   &  Differential Diagnosis \\ 
\hline
\begin{tabular}[c]{@{}l@{}}
female \\ young adult (18 to 40 yrs) \\  few days (2-7 days) \\  cough \\  productive cough \\ malaise \\   fever \\ nose discharge
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}bacterial pneumonia (26.9) \\ influenza (23.4) \\acute sinusitis (22.9)\end{tabular} 
\\ \hline
\begin{tabular}[c]{@{}l@{}}
male \\ middle age (41 to 70 yrs) \\  prolonged (1-4 weeks) \\ foot pain \\ heel pain \\ movement pain \\ walking pain \\ limping
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}plantar fasciitis (38.9) \\ stress fracture (31.5)\end{tabular} 
\\ \hline

\begin{tabular}[c]{@{}l@{}}
female  \\  middle age (41 to 70 yrs)  \\   chronic (> 4 weeks)  \\   urinary urgency  \\   change in bladder habits \\   nocturia  \\   urinary frequency
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}} female  urethritis (32.9) \\ overactive bladder (26.9) \end{tabular} &
\\ \hline
\end{tabular}}
\caption{Examples of clinical cases using simulation from expert system (\S~\ref{sec:simulation}). While the expert systems provide raw scores, these are converted into probabilities through normalization.}\label{fig:sim}
\end{table}
\caption{table caption goes  here}\label{tab: table-label}
\end{minipage}
\end{figure*}




==> sections/simulation.tex <==


%\input{sections/algo}



==> sections/tmp.tex <==


\begin{table*}[]
\centering
\resizebox{\textwidth}{!}{\begin{tabular}{lllll}
\toprule
Findings   & Findings in our feature space & Label  & Learned model & Learned model with COVID                                                                     \\ \hline


\begin{tabular}[c]{@{}l@{}}
30 y/o m \\ 2 day HX of runny
nose \\ sore throat \\ hot,
sweaty \\ mild headache \\cough
with clear sputum \\muscle
aches \\no fever or neck
stiffness 
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
male \\ young adult (18 to 40 yrs) \\brief (6-48 hours)\\nose discharge  \\ sore throat \\  sweating increase \\headache \\productive cough \\ generalized myalgia \\  no fever
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}viral upper respiratory \end{tabular}  &
\begin{tabular}[c]{@{}l@{}}{viral upper respiratory (0.415)}\\ influenza (0.298)  \\ acute sinusitis (0.044)\\ streptococcal pharyngitis (0.028)\\bacterial pneumonia (0.026)\end{tabular} &
\begin{tabular}[c]{@{}l@{}}{viral upper respiratory (0.33)}\\ influenza (0.319)\\COVID-19 (0.058)  \\ acute sinusitis (0.058)\\ streptococcal pharyngitis (0.029)\end{tabular} 
\\ \hline

\begin{tabular}[c]{@{}l@{}}
18 y/o m \\ 3 days severe
headache\\ fever\\
photophobia,\\neck stiffness
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
male \\ young adult (18 to 40 yrs) \\ severe headache \\fever \\ photophobia \\ neck stiffness
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}meningitis \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} bacterial meningitis (0.869) \\ West Nile fever (0.102) \\  Rocky Mountain spotted fever (0.009)\\ influenza (0.005) \\ relapsing fever (0.002)\end{tabular} &
\begin{tabular}[c]{@{}l@{}} bacterial meningitis (0.771) \\ West Nile fever (0.200) \\  Rocky Mountain spotted fever (0.009)\\ influenza (0.005) \\ epidemic myalgic encephalomyelitis (0.002)\end{tabular} 
\\ \hline

\begin{tabular}[c]{@{}l@{}}
-
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
female\\ middle age (41 to 70 yrs)\\thunderclap headache\\headache\\foreign travel history\\nasal congestion
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}} COVID (moderate) \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} cluster headache (0.171) \\ West Nile fever (0.155) \\  dengue (0.107)\\ brain hemorrhage (0.066) \\ migraine (0.065)\end{tabular} &
\begin{tabular}[c]{@{}l@{}} COVID-19 (0.827) \\ West Nile fever (0.026) \\  measles (0.009)\\ cluster headache (0.020) \\ dengue (0.12)\end{tabular} 
\\ \hline


\begin{tabular}[c]{@{}l@{}}
-
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}}
female\\ middle age (41 to 70 yrs)\\generalized myalgia\\headache\\neck stiffness\\hospital personnel(*)
\end{tabular}  &
\begin{tabular}[c]{@{}l@{}} COVID (low) \end{tabular}  &
\begin{tabular}[c]{@{}l@{}} 'West Nile fever (0.356) \\  bacterial meningitis (0.305) \\Saint Louis encephalitis (0.249) \\  Lyme disease: early disseminated (0.069)\\ Rocky Mountain fever(0.005)\end{tabular} &
\begin{tabular}[c]{@{}l@{}} 'West Nile fever (0.308) \\ Saint Louis encephalitis (0.302) \\  COVID (0.235)\\ bacterial meningitis (0.041) \\ Lyme disease: early disseminated (0.036)\end{tabular}  
\\ \hline
\end{tabular}}


\caption{Sample model predictions. Rows 1-2 corresponds to examples from Semigran dataset.  For Semigran cases, we provide the input set of findings from \cite{Semigran}, the corresponding transformation to the findings in the expert system,
the top 5 diseases predicted by model trained without and with the COVID assessment data. Rows 3-4 are examples from the COVID risk assessment
tool. The data format is same as that of Semigran cases, except ``hospital personnel'' in fourth case is a finding only in the model that uses COVID data,
. \TODO{See main text for more details.} }
\label{fig:qual}
\end{table*}




Of closely related, is the work of \cite{ravuri18} which form the premise of our work. 
In that work, an approach was presented the view of expert systems as a data prior: expert systems are generative models of clinical cases that can be used to train a machine learned model for diagnosis that preserves the original properties of the expert systems and also make them more extensible. by showing how they can serve as the starting point to combine expert knowledge with knowledge extracted from other data sources, such as electronic health records.

We take a similar approach in our formulation for incorporating COVID as a potential disease to be considered. We differ from that paper in a few ways:
\begin{itemize}
    \item The simulated cases maintain the uncertainty in the diagnosis, by maintaining a differential diagnosis, as opposed to a single diagnosis.
    \item This enables modeling the output space as a soft multiclass classification
    \item We evaluate the learned models on a dataset that is publicly available. 
    \item Most importantly, we show the timely incorporation of COVID as part of the disease label space for differential diagnosis. The data was attained through a CDC approved assessment flow that identifies if patient needs to be considered for COVID.
\end{itemize}




